Mechanism Learning for Trading Networks

We study the problem of designing mechanisms for trading networks that satisfy four desired properties: dominant-strategy incentive compatibility, efficiency, weak budget balance (WBB), and individual rationality (IR). Although there exist mechanisms that simultaneously satisfy these properties ex post for combinatorial auctions, we prove the impossibility that such mechanisms do not exist for a broad class of trading networks. We thus propose approaches for computing and learning the mechanisms that satisfy the four properties, in a Bayesian setting, where WBB and IR, respectively, are relaxed to ex ante and interim. For computational and sample efficiency, we introduce several techniques, including game theoretical analysis to reduce the input feature space. We empirically demonstrate that the proposed approaches successfully find the mechanisms with the four properties for those trading networks where the impossibility holds ex post.

==> longer_version/abstract.tex <==
%\SW{Trading networks, i.e, firms coming together through bi-lateral contracts in areas such as transportation and supply chain, are becoming increasingly ubiquitous and essential to the world's economy}. \SW{In this work, we} 
We study the problem of designing mechanisms for trading networks
%, \st{where the set of trades and associated payments are determined in a way} 
that satisfy four desired properties: dominant-strategy incentive compatibility, efficiency, weak budget balance (WBB), and individual rationality (IR).  
Although the VCG mechanism can simultaneously satisfy these properties for combinatorial auctions, we prove that such mechanisms do not exist for a broad class of trading networks.  Consequently, we propose approaches for both computing and learning the mechanisms that satisfy the four properties where the \expost{} WBB and IR, respectively, are relaxed to \exante{} and \interim{} in a Bayesian setting.
%\SW{Our contributions therefore include, in addition to the above impossibility result, an automated mechanism design approach for trading networks consisting both of optimization and machine learning formulations for the derivation of such mechanisms.
For computational and sample efficiency, we introduce several techniques, including game theoretical analysis to reduce the input feature space.
Empirically, we demonstrate the effectiveness of the proposed approaches in designing mechanisms for those trading networks where the impossibility holds \expost{}.

%July 4, 2022: AAAI-23 web site open for author registration
%July 11, 2022: AAAI-23 web site open for paper submission
%ugust 8, 2022: Abstracts due at 11:59 PM UTC-12
%August 15, 2022: Full papers due at 11:59 PM UTC-12

